Extract-and-Adaptation Network for 3D Interacting Hand Mesh Recovery

Understanding how two hands interact with each other is a key component of accurate 3D interacting hand mesh recovery. However, recent Transformer-based methods struggle to learn the interaction between two hands as they directly utilize two hand features as input tokens, which results in distant token problem. The distant token problem represents that input tokens are in heterogeneous spaces, leading Transformer to fail in capturing correlation between input tokens. Previous Transformer-based methods suffer from the problem especially when poses of two hands are very different as they project features from a backbone to separate left and right hand-dedicated features. We present EANet, extract-and-adaptation network, with EABlock, the main component of our network. Rather than directly utilizing two hand features as input tokens, our EABlock utilizes two complementary types of novel tokens, SimToken and JoinToken, as input tokens. Our two novel tokens are from a combination of separated two hand features; hence, it is much more robust to the distant token problem. Using the two type of tokens, our EABlock effectively extracts interaction feature and adapts it to each hand. The proposed EANet achieves the state-of-the-art performance on 3D interacting hands benchmarks. The codes are available at https://github.com/jkpark0825/EANet.

==> sections/figures/tsne.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/firstshow/overall_label.pdf}
    \\
    \includegraphics[width=0.22\linewidth]{figures/tsne/input_asym1.png}
    \includegraphics[width=0.22\linewidth]{figures/tsne/tsne_asym1.pdf}
    \includegraphics[width=0.22\linewidth]{figures/tsne/input_asym3.jpg}
    \includegraphics[width=0.22\linewidth]{figures/tsne/tsne_asym3.pdf}
    % \includegraphics[width=\wp]{figures/tsne/tsne_paper.pdf}
    \vspace{-2mm}
    \caption{\textbf{Visualization of token distribution with t-SNE~\cite{van2008visualizing}.} 
    t-SNEs are drawn with tokens from a single input image (left).
    Our \textcolor{simtoken_red}{SimToken} and \textcolor{jointoken_green}{JoinToken} are in homogeneous space, while \textcolor{left_hand_orange}{left} and \textcolor{right_hand_blue}{right} hand features are in heterogeneous spaces.}
    \label{fig:tsne}
    \vspace{-3mm}
\end{figure}

==> sections/tables/interhand.tex <==
\begin{table}[t]
    \centering
    \resizebox{1.\linewidth}{!}{
    \begin{tabular}{c|ccc|ccc|c}
        \toprule
         & \multicolumn{3}{c|}{MPJPE} & \multicolumn{3}{c|}{MPVPE}  & MRRPE\\
        Methods & Single & Two & All & Single & Two & All & Two\\
        \midrule
        Zhang~\etal~\cite{zhang2021interacting} & - & 13.07 &  - & - & 13.95 & - & -\\
        LWA-HAND~\cite{di2022lwa} & - & 12.56 & - &  - &  12.37 & - &  -\\
        Intaghand~\cite{li2022interacting} & - & 8.79 & - &  -  &  \textbf{9.03} &  - &  -\\
        \textbf{Link2Hands~(Ours)} & 5.56 & \textbf{7.70} & 6.63 & 7.38 & 11.54 & 8.92 & 28.54 \\
        \midrule
        Pose2Pose~\cite{moon2022accurate} & 13.54 &  16.82 &  15.18 &  - &  - &  - & 37.47\\
        InterNet~\cite{moon2020interhand2} & 12.13 & 16.01 & 14.20 &  - &  - &  - & 32.60\\
        Fan~\etal~\cite{fan2021learning} & 11.32 & 15.57 & - &  - &  - &  - &  30.51\\
        Keypoint Transformer~\cite{hampali2022keypoint} & \textbf{11.08} & 15.33 & \textbf{13.41} &  16.21 &  30.84 &  22.41 & 30.87\\
        \textbf{Link2Hands~(Ours)} & 11.66 & \textbf{15.16} & \textbf{13.41} &  \textbf{10.99} & \textbf{14.48} &  \textbf{12.28} & \textbf{28.54} \\
        \bottomrule
    \end{tabular}}
    \caption{\textbf{Quantitative comparison with state-of-the-art methods on Interhand2.6M dataset.} For fair comparison, we report metrics after scale alignment in top, and metrics befor any alignment process in bottom.}
    \vspace{-5mm}
    \label{tab:interhand}
\end{table}
